Transferability Metrics for Selecting Source Model Ensembles

We address the problem of ensemble selection in transfer learning: Given a large pool of source models we want to select an ensemble of models which, after fine-tuning on the target training set, yields the best performance on the target test set. Since fine-tuning all possible ensembles is computationally prohibitive, we aim at predicting performance on the target dataset using a computationally efficient transferability metric. We propose several new transferability metrics designed for this task and evaluate them in a challenging and realistic transfer learning setup for semantic segmentation: we create a large and diverse pool of source models by considering 17 source datasets covering a wide variety of image domain, two different architectures, and two pre-training schemes. Given this pool, we then automatically select a subset to form an ensemble performing well on a given target dataset. We compare the ensemble selected by our method to two baselines which select a single source model, either (1) from the same pool as our method; or (2) from a pool containing large source models, each with similar capacity as an ensemble. Averaged over 17 target datasets, we outperform these baselines by 6.0% and 2.5% relative mean IoU, respectively.

==> Transferability Metrics for Selecting Source Model Ensembles- CVPR 2022/0_abstract.tex <==

\begin{abstract}
   We address the problem of ensemble selection in transfer learning: Given a large pool of source models we want to select an ensemble of models which, after fine-tuning on the target training set, yields the best performance on the target test set. Since fine-tuning all possible ensembles is computationally prohibitive, we aim at predicting performance on the target dataset using a computationally efficient transferability metric.
   %
   We propose several new transferability metrics designed for this task and evaluate them in a challenging and realistic transfer learning setup for semantic segmentation:
   we create a large and diverse pool of source models by considering 17 source datasets covering a wide variety of image domain, two different architectures, and two pre-training schemes.
   Given this pool, we then automatically select a subset to form an ensemble performing well on a given target dataset.
   %
   We compare the ensemble selected by our method to two baselines which select a single source model, either (1) from the same pool as our method; or (2) from a pool containing large source models, each with similar capacity as an ensemble.
   Averaged over 17 target datasets, we outperform these baselines by 6.0\% and 2.5\% relative mean IoU, respectively.
   
\end{abstract}



==> Transferability Metrics for Selecting Source Model Ensembles- CVPR 2022/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

In transfer learning we want to re-use knowledge previously learned on a source task to help learning a target task. The most common form of transfer learning in computer vision is to pre-train a single source model on the generic ILSVRC dataset~\cite{azizpour15pami, chu16eccv, girshick15iccv, he17iccv, huh16neurips, kornblith19cvpr, shelhamer16pami, zhou19arxiv} and then fine-tune it on the target dataset. However, often a more domain-specific approach can lead to better results \cite{mensink21arxiv, ngiam18arxiv, yan20cvpr}.
Hence, it is beneficial to have a large pool of diverse source models such that it contains models suited for many different target tasks. The problem then becomes: how can we automatically and efficiently select good source models for a given target task?

Recently, transferability metrics were introduced to address this problem~\cite{bao19icip, nguyen20icml, li21cvpr, you21icml, tan21cvpr, tran19iccv}. The general goal is to select a single source model which, after fine-tuning on the target training set, yields the best performance on the target test set. Transferability metrics enable to select this model efficiently without carrying out expensive fine-tuning on the target training set.

While previous transferability metrics consider selecting a single source model, in this paper we aim at selecting a subset containing multiple source models to form an {\em ensemble}.
Ensembles are a general technique used to improve model accuracy, out-of-distribution robustness, and to estimate uncertainty \cite{breiman96ml, dietterich00springer, freund96icml, fort19arxiv, krogh95nips, lakshminarayanan17neurips, ovadia19nips, wang20arxiv}.
Furthermore, by aggregating multiple source models, we can combine knowledge coming from multiple source datasets and image domains, which may be beneficial for a particular target task.
%
Hence, in this paper we extend previous work on transferability by proposing several transferability metrics designed for {\em ensemble selection}.

To evaluate ensemble selection we introduce a challenging experimental setup.
We consider semantic segmentation as a task, with a truly diverse pool of source models, as we train them on 17 complete datasets spanning a wide variety of images domains, while also varying their model architectures and pre-training schemes (Fig.~\ref{fig:pipeline}).
In contrast, previous works typically
focus on image classification~\cite{bao19icip, nguyen20icml, li21cvpr, you21icml, tan21cvpr, tran19iccv},
consider a narrower range of at most 4 source datasets \cite{tan21cvpr,nguyen20icml,you21icml,li21cvpr},
and often generate multiple datasets artificially by sampling different subsets of classes out of a single actual dataset~\cite{bao19icip, nguyen20icml, tan21cvpr, tran19iccv}.

To summarize, we make the following contributions:
%
(1) We design transferability metrics for \emph{ensemble} selection.
%
(2) We consider a challenging application scenario on semantic segmentation featuring a large and truly diverse pool of source models.
%
(3) We compare the ensemble selected by our method to two baselines which select a single source model, either from the same pool as our method; or from a pool containing large source models, each with similar capacity as an ensemble.
Averaged over 17 target datasets, we outperform these baselines by 6.0\% and 2.5\% relative mean IoU, respectively (Sec. \ref{sec:ensemble_selection_results}).



==> Transferability Metrics for Selecting Source Model Ensembles- CVPR 2022/2_related_work.tex <==
\section{Related Work} \label{related_work}
\label{sec:related-works}

\para{Transfer Learning.}
The most common form of transfer learning in computer vision is to pre-train a model on ILSVRC'12~\cite{dosovitskiy20arxiv, kolesnikov20eccv}, and fine-tune it on the target dataset.
Several works extend this to using a larger source dataset such as ImageNet21k (9M images), JFT-300M (300M images) \cite{dosovitskiy20arxiv, kolesnikov20eccv, mustafa20arxiv}, or Open Images (1.7M images) \cite{yan20cvpr}.
Other works consider self-supervised pre-training, enabling the use of unlabeled source datasets (\eg~\cite{he20cvpr, chen21cvpr, chen20icml, islam21iccv, li21iccv}).

% JASPER: Reordered such that Taskonomy is last, which enabled the tail task-relatedness predictions.
Several studies explore in-depth under which circumstances transfer learning works.
Mensink et al.~\cite{mensink21arxiv} study transfer learning across datasets with vastly different image domains and multiple visual tasks.
Mustafa et al.~\cite{mustafa21arxiv} studies transfer learning in medical imaging.
Finally, Taskonomy~\cite{zamir18cvpr} establishes relationships between visual tasks (\eg semantic segmentation, depth prediction, etc.).
Following the success of Taskonomy, several works investigate whether visual task relatedness can be predicted~\cite{dwivedi19cvpr, song19neurips, song20cvpr, dwivedi20eccv, bolya21neurips} rather than calculated by brute force~\cite{zamir18cvpr}.

% Several studies explore in-depth under which circumstances transfer learning works.
% Taskonomy~\cite{zamir18cvpr} establishes relationships between visual tasks (\eg semantic segmentation, depth prediction, etc.). % 3D keypoint prediction).
% Mensink et al.~\cite{mensink21arxiv} study transfer learning across datasets with vastly different image domains and multiple visual tasks, while
% Mustafa et al.~\cite{mustafa21arxiv} focus on the medical imaging domain.


% Less shortened version. DO NOT REMOVE FROM TEX.!
% \jasper{This paragraph is still way too long.}
% \jasper{Shortened, removed negativity.} Taskonomy~\cite{zamir18cvpr} is a landmark work towards understanding relationships between different visual tasks such as semantic segmentation, depth prediction, 3D keypoint prediction, etc. They establish these relationships by using a single dataset with annotations for all visual tasks.
% \cite{mensink21arxiv} aim to understand which factors influence transfer learning. They perform a large-scale exploration across many datasets with vastly different image domains (\eg consumer, driving, indoor) and across different visual tasks (semantic segmentation, object detection, depth estimation, keypoint detection).
% In~\cite{mustafa20arxiv} they investigate the benefits of transfer learning to the medical imaging domain.
% \jasper{I don't think the neural data server fits as an analysis paper.}

Only a few works conduct transfer learning from multiple source datasets at the same time.
Liu et al.~\cite{liu19iclr} train a student model using knowledge from
%\vitto{added `distillation', I hope it's true}
%\jasper{No, it is not; it is a strange paper: they merge features from teachers and feed this to the student. Intuitively, this pushes later layers to consume features similar to that of the teacher, which apparently works. Anyway, I kept it a bit vague on purpose}
multiple teachers (\ie source models), which is expensive in both memory and computation.
Zoo-Tuning \cite{shu21icml} learns to aggregate the parameters of multiple source models into a target model. This requires storing all source models in memory during training, limiting scalability.
In contrast, we select an ensemble from a large pool of source models in a computationally and memory efficient manner.

\para{Transferability Metrics.}
Recently, several papers introduced transferability metrics.
% \changed{\cite{dwivedi19cvpr, song19neurips, song20cvpr, dwivedi20eccv, bolya21neurips} focus at predicting visual task relatedness and evaluate their methods on the Taskonomy benchmark.}
% methods which aim to predict how well a source model will transfer to a target task 
H-score \cite{bao19icip} measures the discriminativeness of source model features on the target task in terms of inter-class and intra-class variance. 
LEEP~\cite{nguyen20icml} measures how well a classifier built on top of source model predictions performs on the target task.
$\mathcal{N}$LEEP~\cite{li21cvpr} trains a Gaussian Mixture Model (GMM) on top of source model features. Then it measures how well a classifier built on top of these GMM predictions performs on the target task. 
LogME~\cite{you21icml} estimates accuracy on the target task based on a formulation which integrates over all possible linear classifiers built on top of the source model features.
OTCE~\cite{tan21cvpr} applies a source model to extract image features from both the source and target dataset. Then it uses optimal transport between these features to calculate domain difference and task difference. 
Finally, NCE~\cite{tran19iccv} considers a more restrictive setting where the source and target datasets consist of identical images. Their method uses conditional entropy between ground truth source and target labels, which avoids training models and is thus computationally efficient.

To put our work in context:
(1) Instead of selecting a single source model~\cite{bao19icip, nguyen20icml, li21cvpr, you21icml, tan21cvpr}, we do \emph{ensemble} selection.
(2) Instead of image classification~\cite{bao19icip, nguyen20icml, li21cvpr, you21icml, tan21cvpr, tran19iccv}, we address semantic segmentation.
(3) We consider a larger variety of source datasets than previous works (17 vs at most  4~\cite{tan21cvpr}).
(4) We consider complete datasets, whereas previous works often sample different subsets of classes out of a single actual dataset~\cite{bao19icip, nguyen20icml, tan21cvpr, tran19iccv}.
%(5) Like~\cite{li21cvpr, you21icml}, we focus on the most practical application for transfer learning: given one target dataset, we select which source models to use out of a pool. Other works~\cite{bao19icip, nguyen20icml, tan21cvpr, tran19iccv} focus instead on the converse setting: given one source, determine which target datasets it would help the most, out of a pool of targets.

%\jasper{Perhaps the next paragraph is still a bit too verbose for the related work.}
%All these transferability metrics were introduced to select a single source model for a target dataset \andrea{same argument as above}. In this paper we introduce transferability metrics which select an \emph{ensemble} of source models. In addition, previous works typically address image classification and create artificial source and target datasets by subsampling existing datasets according to a subset of labels \andrea{what about 'by sampling different sets of labels from existing datasets'?}. Instead, in this paper we address semantic segmentation in a realistic transfer learning scenario where we consider 17 complete datasets which span a wide variety of image domains. Since our setting has high computational demands, both in terms of ensemble selection and semantic segmentation, in this paper we choose to extend LEEP~\cite{nguyen20icml}. \andrea{do we need to say that we start from leep here? Also from the metrics it is not clear that is the most memory and (maybe) computationally efficient}


\para{Ensemble of Models.} \label{para:ensemble}
Ensembling machine learning models is a classical method for increasing accuracy~\cite{breiman96ml,dietterich00springer,freund96icml,hansen90pami,krogh95nips,lee15arxiv}, where having diverse models is typically important. More recently, ensembles of deep neural network have been studied in the context of uncertainty estimation and out-of-distribution robustness~\cite{allingham21arxiv, fort19arxiv, lakshminarayanan17neurips, ovadia19nips}.
%
%In this paper we address the problem selecting a ensemble of source models that will perform best at transfer learning to a target dataset. We propose new transferability metrics for this problem.



%%%%%%%%%%%%%%%%%%%%%%%%
% END OF PARAGRAPH.
%%%%%%%%%%%%%%%%%%%%%%%%

% Several works propose analytical solutions to select a source to transfer from. H-score \cite{bao19icip} uses statistical and information theoretic principles to compute a transferability metric. Better transferability is measured as a result of higher inter-class variance and lower feature redundancy. NCE \cite{tran19iccv} proposes a method based on the conditional entropy between the label assignment of the two models. It does not require any training, but it assumes that the source and target data share the same input examples. LEEP \cite{nguyen20icml} constructs an empirical predictor from the estimation of the joint label distribution between target and source space. The metric has a direct interpretation, as it consists of the average log-likelihood of the empirical predictor.

% More recently, several papers propose transferability metrics that can be applied to broader scenarios. \cite{you21icml} proposes a probabilistic approach through logarithm of maximum evidence (LogME). They show improved results over prior methods, and they extend the application of transferability metrics to unsupervised pre-trained models and regression tasks. OTCE \cite{tan21cvpr} extends the previous experimental settings to cross-domain and cross-dataset. It uses optimal transport to evaluate the domain difference of 2 datasets. Then, they compute a task difference measure from the empirical joint probability distribution between target and source label sets. Finally they obtain their metric as a weighted combination of domain and task difference.  Additionally, they provide a short study for multi-source transfer learning, where they use the OTCE score to weight the aggregation of the features. However, their purpose was not to build a metric designed to select a combination from a big pool of source models, in fact they use only 4 source models and they apply OTCE per source independently, without modelling relationships between sources.

% Despite the advances towards a more applicable transferability metric and broader experimental setup, there are various areas that have not being explored. In our work we target the semantic segmentation task, and the multi source setting, where no other work propose solutions. We validate our work on a total of 68 source models, and 17 target datasets from 6 image domains. This consists of the most diverse experimental setup used to apply a transferability metric.

% \jasper{Deprecated from here.}
% \jasper{We need more citations here.}
% Ensemble learning is an established machine learning technique \cite{zhou19crc}, landmark works include Bagging \cite{breiman96ml}, Boosting \cite{freund97jcss} and AdaBoost \cite{schapire13springer}. Recently, ensembles of neural networks have been studied as a way to improve accuracy, uncertainty and out-of-distribution robustness \cite{fort19arxiv}, and as an efficient alternative to state-of-the-art single models, even for structured semantic segmentation tasks \cite{wang20arxiv}.
% 
% A good ensemble is composed by individual members that are both accurate and diverse. \cite{krogh95nips} decomposes the ensemble error $E$ as:
% \begin{equation}
%     E=\Bar{E}-\Bar{A}
% \end{equation}
% $\Bar{E}$ is the average error of individual models, while $\Bar{A}$ denotes the average ambiguity, or diversity, among the members. The equation is a general guidance towards the ensemble construction. To create ensemble diversity, a basic approach is to manipulate the data. For example, Bagging \cite{breiman96ml} uses bootstrap sampling \cite{tibshirani93msap}, while AdaBoost introduces importance sampling \cite{schapire13springer}. When it comes to the application of ensemble models to deep learning, weights random initialization prevailed as a good approach to diversify neural networks \cite{fort19arxiv}.
% 
% The diversity-accuracy trade off of ensemble members has been shown to be a fundamental reason of their success. However, the majority of these studies focus on simple sources of diversity, and are usually limited to classification tasks \cite{fort19arxiv}. In our work we envision having a naturally diverse set of source models, exploiting 3 sources of diversity: model architecture, pre-training strategy and source dataset. Additionally, we target transfer learning for semantic segmentation tasks, and we propose new approaches for measuring transferability from ensemble of source models.


\begin{comment}
\jasper{Overview of experimental setups for the various papers.}

OTCE~\cite{tan21cvpr}: Experiments only involve target dataset selection. In particular, they consider either DomainNet or Office31, both of which are composite datasets which comprise a variery of domains. For each experiment, they train a single source model on a given domain (e.g. ClipArt in DomainNet). Then they generate multiple target datasets: for each domain they sample 100 classification tasks by sampling different label sets. 
Afterwards, they turn the experiment into a source-model selection problem: for each of the target tasks (100 per domain), they consider 4 source models and determine whether their method selects the best one. They report percentage in which their method is correct.
They also have a mini-experiment on using OTCE to do feature fusion, but *not* for source model selection as we do.

LogME~\cite{you21icml}: They consider source model selection by pre-training 10 different architectures on ILSVRC'12. 
Then (1) they each time consider a single target dataset out of 9 commonly used datasets.
Then (2) they do the same but for a single regression task.
Then (3) they do the same but using source models trained using self-supervised pre-training (which cannot be used by LEEP/NCE, since no predictions (LEEP) or source labels (NCE) are available.
Then (4) they do source model selection for language tasks (using available pre-trained architectures and published transfer learning performance).

LEEP~\cite{nguyen20icml}: They do target dataset selection. They consider ResNet18 and ResNet20. They consider ImageNet->Cifar100 and Cifar10->Cifar100. For all four experiments they consider a single source, and subsample target datasets by subsampling labels (randomly between 2-100 labels).
\andrea{on 5.7 they do source model selection, 9 different model architectures pre-trained on ImageNet, they test just on CIFAR100}

H-score~\cite{bao19icip}: They do target dataset selection. They consider a pre-trained ResNet50 on ImageNet. Then they sample randomly 20k images from Cifar-100 to do target dataset selection. They do also separate experiments sampling 5k, 10k, 30k, and 50k images.
They also do source selection on the Taskonomy dataset. They suspiciously only used part of this dataset, and show positive correlations (without any baseline, since they were the first). Finally, they looked at fusing features of two models (!).

NCE~\cite{tran19iccv}: Their method only works on the same images with different label spaces. In their evaluation, they use three different attribute datasets: Celeb Faces Attributes (CelebA), Animals with Attributes V2 (AwA2), and Caltech-UCSD Birds 200. Each time they consider a single attribute, and predict how it transfers to each other attribute. So in a way they are also doing target dataset selection.

Ranking Neural Checkpoints~\cite{li21cvpr}: They perform source model selection. In each experiment they consider a single target dataset; Caltech-101, Flowers102, Sun397, and Patch Camelyon. They consider three different groups of source models. 
In group 1, they start from 16 ResNet50s: 14 of those are pre-trained on ImageNet using a variety of strategies. Examples are JigSaw, Rotation, exemplar, VAE variants, GAN variants, semi-supervised variants which combine self-supervised learning on all data with fully supervised learning on either 10\% of 100\% of the data. Additionally, they train ResNet50 on INaturalist and Places365.
In Group 2, they consider fully supervised ResNet50 on ImageNet, Inaturalist, and places365, but take checkpoints directly after each learning-rate decay. In their learning rate schedule, the reduce the learning rate 3 times. Since they also take the final checkpoint, this results in 4 checkpoints per model. (12 source models in total).
In Group 3, they consider different architectures: 2 ResNet variants, 4 Inception variants, InceptionResNetV2, 6 MobileNet variants. They are all trained fully supervised on ImageNet.
In the appendix, they have an experiment on Pascal VOC object detection, and cityscapes instance segmentation, starting from 4 source models only. These are all ResNet50 variants pre-trained on ImageNet using MoCoV1, MoCoV2, MoCoV3, and fully supervised.

\end{comment}

==> Transferability Metrics for Selecting Source Model Ensembles- CVPR 2022/3_method.tex <==
\section{Methods} \label{sec:methods}

We consider the problem of source model ensemble selection for semantic segmentation.
Given $N$ source models and a target dataset, the goal is to select an \emph{ensemble} of source models which, after fine-tuning on the target training set, yields the best performance on the target test set. Since fine-tuning all possible ensembles is too computationally expensive, we predict performance on the target dataset using a computationally efficient transferability metric.

\cref{preparing_source_models} discusses what makes for a good pool of source models and describes how we construct this pool. 
\cref{metric-semantic-segmentation} describes our setup to work with transferability metrics in semantic segmentation tasks.
\cref{leep-single} describes LEEP~\cite{nguyen20icml}, a transferability metric for single-source selection. 
We use this as a starting point in~\cref{metric-multi-source} to define our four transferability metrics for \emph{ensemble} selection.

% OLD VERSION BEFORE CAMREADY
% \cref{preparing_source_models} discusses what makes for a good pool of source models and describes how we construct such a pool. 
% \cref{metric-semantic-segmentation} briefly describes how we setup the data for semantic segmentation instead of the image classification task considered in previous works on transferability~\cite{bao19icip, li21cvpr, nguyen20icml, you21icml, tan21cvpr, tran19iccv}.
% In \cref{leep-single} we describe LEEP~\cite{nguyen20icml}, a transferability metric for single-source selection. 
% We use this as a starting point in~\cref{metric-multi-source} to define our four transferability metrics for \emph{ensemble} selection.


\subsection{Preparing source models} \label{preparing_source_models}

We want to create a pool with a large variety of source models for three reasons:
(1) this increases the chance that for any given target dataset there exists at least one good source model.
(2) we need bad source models to verify that our transferability metrics correctly select good source models while discarding bad ones.
(3) an ensemble can only outperform its individual members if they are diverse (and therefore complementary)~\cite{bian21ieee, dietterich00springer, freund96icml, hansen90pami, krogh95nips}.
Hence, we construct our source model pool by incorporating diversity in three ways: we use 17 different source datasets, two model architectures and two pre-training strategies.
Tab.~\ref{tab:setup_comparison} summarizes how this setup compares to related work.

\begin{table}[t!]
\footnotesize	%\scriptsize	
\vspace{-0.6cm}
  \centering
  \setlength\tabcolsep{2.8pt}
  \begin{tabular}{l | c c c c c c}
    \toprule
     & Ours & Ours & LEEP & LogME & OTCE & $\mathcal{N}$LEEP \\
     & \cref{sec:ensemble_selection} & \cref{sec:evaluate-metrics} & \cite{nguyen20icml}
     & \cite{you21icml} & \cite{tan21cvpr} & \cite{li21cvpr} \\
    \midrule
     \# source datasets & 17 & 10-15 & 1 & 1 & 4 & 3\\
     \# pre-training schemes & 2 & 1-2 & 1 & 1 & 1 & 4\\
     \# model architectures & 2 & 1-2 & 9 & 10 & 1 & 13\\
     \# source models & 68 & 15 & 9 & 10 & 4 & 41\\
    \midrule
    \# candidates & 41K & 455 & 9 & 10 & 4 & 41 \\
  \end{tabular}
  \caption{Comparing our experimental setup (see Sec. \ref{sec:evaluate-metrics} and \ref{sec:ensemble_selection}) to previous works on cross-dataset source selection. We compare the diversity of source models in terms of the number of source datasets, pre-training schemes, and model architectures.
  The last row denotes the number of candidate source models (or ensembles in our case) that are in the pool for a given target dataset. For~\cite{li21cvpr, nguyen20icml, tan21cvpr, you21icml} we consider their largest source selection experiment.}
  \label{tab:setup_comparison}
  \vspace{-0.4cm}
\end{table}


\para{Source datasets.}
The image domain is one of the most important factors to influence whether transfer learning will succeed~\cite{ngiam18arxiv, mensink21arxiv, pan09ieee}, and therefore we want to cover a wide array of image domains. Furthermore, the most natural way to perform transfer learning is to consider each dataset as a whole (rather than subsampling a dataset to simulate dataset variations~\cite{bao19icip, nguyen20icml, tan21cvpr, tran19iccv}). 
Therefore, we adopt the realistic cross-dataset transfer learning setup for semantic segmentation by~\cite{mensink21arxiv}: 17 source datasets from 6 image domains (consumer photos, driving, aerial, indoor, underwater, synthetic; Tab.~\ref{tab:datasets}).
While this setup was defined in~\cite{mensink21arxiv}, that work did not explore any transferability metric.


\para{Model architectures.}
We consider two semantic segmentation architectures, each with a backbone and a linear classification layer.
As the first backbone we choose HRNetV2~\cite{wang20pami}, a high-resolution alternative to ResNet. It maintains parallel feature representations at different resolutions, which helps dense prediction tasks~\cite{lambert20cvpr,mensink21arxiv,wang20pami}. As ensembles contain multiple models, we choose a light-weight version: HRNetV2-W28 (23M parameters).

\begin{table}[pt]
\vspace{-0.6cm}
    \centering
    \resizebox{0.5\textwidth}{!}{
        % To hide the number column: replace l with H
        \begin{tabular}{llcc}\toprule
        Dataset                      & Domain  & \# classes  & \# train images  \\
        \midrule
        Pascal Context~\cite{mottaghi14cvpr}  & Consumer              & 60        & 5K \\
        Pascal VOC~\cite{pascal-voc-2012} & Consumer              & 22   &  10K \\
        ADE20K~\cite{zhou17cvpr}      & Consumer              & 150   &   20K \\
        COCO Panoptic~\cite{caesar18cvpr, lin14eccv, kirillov19cvpr}       & Consumer              & 134 & 118K \\
        KITTI~\cite{alhaija18ijcv}   & Driving & 30 & 150 \\
        CamVid~\cite{brostow09prl}    & Driving  & 23 & 367 \\
        CityScapes~\cite{cordts16cvpr}    & Driving  & 33   & 3K \\
        India Driving Dataset (IDD)~\cite{varma19wacv} & Driving & 35 & 7K \\
        Berkeley Deep Drive (BDD)~\cite{yu20cvpr} & Driving & 20 & 7K \\
        Mapillary Vista Dataset~\cite{neuhold17cvpr} & Driving & 66 & 18K \\
        ISPRS~\cite{rottensteiner14isprs}  & Aerial & 6 & 4K \\
        iSAID~\cite{waqas2019isaid, xia18cvpr} & Aerial     & 16 & 27K \\
        SUN RGB-D~\cite{song15cvpr} & Indoor & 37 & 5K \\
        ScanNet~\cite{dai17cvpr} & Indoor & 41 & 19K \\
        SUIM~\cite{islam2020suim} & Underwater & 8 & 1525 \\
        vKITTI2~\cite{cabon20arxiv, gaidon16cvpr} & Synthetic driving & 9 & 43K \\
        vGallery~\cite{weinzaepfel19cvpr} & Synthetic indoor & 8 & 44K \\
        \bottomrule
        \end{tabular}
    }
    \caption{Semantic segmentation datasets used in our paper.}
    \label{tab:datasets}
    \vspace{-.4cm}
\end{table}

As the second backbone, we adopt a high-resolution variant of ResNet50~\cite{he16cvpr}.
%
First, we remove the downsampling operations in the last two ResNet blocks while increasing the dilation rate~\cite{wu19pr}.
%
Second, we add an upsampling layer using 5 parallel atrous convolutions with different dilation rates, which enlarges the field of view of the filters without compromising on spatial resolution \cite{chen17pami}.
%
Finally, we remove the last four layers of the last ResNet block to make this backbone have the same number of parameters as HRNetV2-W28 (we call this model ResNet23M).
As all ensembles we build contain the same number of source models, this ensures that they also have the same number of parameters, enabling a fair comparison between them.

% ORIGINAL VERSION BEFORE CAMREADY; shortened above
% As the second backbone, we adopt a variant of ResNet50~\cite{he16cvpr}. As its low-resolution predictions generally result in poor performance, we create a higher-resolution version by incorporating two ideas from~\cite{chen17pami,wu19pr}.
% %
% First, we remove the downsampling operations in the last two ResNet blocks while increasing the dilation rate accordingly~\cite{wu19pr}.
% %
% Second, we add an upsampling layer using 5 parallel atrous convolutions with different dilation rates, which is a computationally efficient way to enlarge the field of view of filters without compromising on spatial resolution \cite{chen17pami}.
% %
% Finally, we remove the last four layers of the last ResNet block to make this backbone have the same number of parameters as HRNetV2-W28 (we call this model ResNet23M).
% As all ensembles we build contain the same number of source models, this ensures that they also have the same number of parameters, enabling a fair comparison between them.




\para{Pre-training schemes.}
Fully supervised pre-training on ILSVRC'12 generally benefits semantic segmentation \cite{mensink21arxiv,shelhamer16pami}.
Furthermore, self-supervised pre-training is making rapid progress and can even outperform fully supervised pre-training~\cite{li21iccv,islam21iccv}.
%in some experiments~\cite{li21iccv,islam21iccv}.
To maximize model diversity, we create two variants of each source model by using two types of ILSVRC'12 pre-trained weights: fully supervised and using the self-supervised SimCLR method~\cite{chen20icml}.


% Fully supervised pre-training  for image classification on ILSVRC'12 generally benefits semantic segmentation \cite{mensink21arxiv,shelhamer16pami}.
% Furthermore, self-supervised pre-training is making rapid progress and can even outperform fully supervised pre-training
% in some experiments~\cite{li21iccv,islam21iccv}.
% To maximize model diversity, we create two variants of each source model by using two types of ILSVRC'12 pre-trained weights: fully supervised and using the self-supervised SimCLR method~\cite{chen20icml}.


\para{Training source models.} \label{para:training-setup}
We have 17 source datasets, two architectures, and two pre-training schemes.
We train a source model for each combination, i.e. 68 in total (details in the Appendix B). These models are trained only once and reused in all experiments.

% We train using a pixel-wise cross-entropy loss, optimized by SGD with momentum \cite{qian99nn}.
% We use 8 Google Cloud TPUs v3 with synchronized batch norm and batch size 32.
% We decrease the learning rate by $10\times$ after $2/3$ of the total training steps.
% For each model, we tune the initial learning rate and number of training steps on the source dataset.



\subsection{Setting up for semantic segmentation} \label{metric-semantic-segmentation}

In most previous works \cite{you21icml, nguyen20icml, tan21cvpr, bao19icip, tran19iccv, li21cvpr}, a transferability metric is primarily applied to image classification, where an image is associated to one label.
In semantic segmentation instead we have predictions at the pixel level,
and therefore we consider for each pixel $x_i$ and its ground-truth label $y_i$ as an individual example $(x_i, y_i)$.

The number of datapoints in semantic segmentation is approximately 6 orders of magnitude higher than in image classification. To reduce the computational cost, we sample 1000 pixels per image to calculate each transferability metric. 
% REMOVED CamReady: This reduces the total computation by 3 orders of magnitude.
%
Furthermore, semantic segmentation datasets often have large class imbalance, which can negatively affect results.
% REMOVED CamReady: especially since one evaluates typically using mean IoU~\cite{cordts16cvpr, everingham15ijcv, lambert20cvpr, shelhamer16pami}, which considers each class as equally important.
Therefore, we sample pixels inversely proportionally to the frequency of their class labels in the target dataset.



\subsection{LEEP as single-source transferability metric}\label{leep-single}

We want a transferability metric suitable for selecting an ensemble of models for semantic segmentation.
We start from LEEP~\cite{nguyen20icml}, which is based on probability distributions, for several reasons.
First, both per-pixel predictions and ensemble selection increase computational and memory complexity compared to the usual image classification and single-source selection.
LEEP is computationally cheap, requiring just a single forward pass of the target training set through the source model, without additional training. Second, LEEP is memory-efficient as it stores predictions instead of features as opposed to alternative metrics~\cite{you21icml, tan21cvpr, bao19icip}.
Finally, starting from LEEP we can derive clear mathematical formulations for the multi-source setting.

LEEP calculates a transferability score between a single source model $s$ and a target training set $\mathcal{D}_t$, containing a set of training samples $(x_i, y_i)\in\mathcal{D}_t$.
Applying $s$ to a target sample produces the probability $p_{\textrm{s}}(z|x_i)$, for each source class $z$ in the source label space $\mathcal{Z}$.
%
The core idea of LEEP is to associate predictions in the source label space $\mathcal{Z}$ to predictions in the target label space $\mathcal{Y}$.
To do so, we apply $s$ to all samples in $\mathcal{D}_t$, and then compute the empirical joint distribution $\hat{P}(y,z)$ measuring co-occurrences between all pairs of labels $(y,z) \in \mathcal{Y} \times \mathcal{Z}$. 
%\tm{Alternative: 
%To do so, we estimate $p_s(z|x_i)$ for each image-ground truth pair $(x_i, y_i)$ in $\mathcal{D}_t$ and aggregate the scores in row $y_i$ of a $\mathcal{Y} \times \mathcal{Z}$ matrix to estimate the empirical joint distribution $\hat{P}(y,z)$.}\jasper{IMHO the matrix is more of an implementation detail rather than meaning, so I would leave it as is.}

Next, we can calculate the empirical conditional distribution $\hat{P}(y|z)$ as $\frac{\hat{P}(y,z)}{\hat{P}(z)}$.
%
Given the source model $s$, we can now construct a classifier, called  \textbf{E}xpected \textbf{E}mpirical \textbf{P}redictor (EEP): 
%
\begin{equation}
  p_s(y_i|x_i) = \sum_{z\in \mathcal{Z}}{\hat{P}(y_i|z) p_{\textrm{s}}(z|x_i)}
  \label{eq:eep}
\end{equation}
%
Here $p_s(y_i|x_i)$ is the probability that model $s$ assigns to the ground-truth label $y_i$ at pixel $x_i$.
LEEP is defined as the log-average of the predictor over $\mathcal{D}_t$:
%
\begin{equation}
  %\mathrm{LEEP} = \frac{1}{n}\sum_{i=1}^{n}\log\left(p_s(y_i|x_i)\right)
  \mathrm{LEEP} = \frac{1}{n}\sum_{i=1}^{n}\log p_s(y_i|x_i)
  \label{eq:leep}
\end{equation}
%
We can see that LEEP measures how well the constructed classifier EEP performs on $\mathcal{D}_t$, where better transferability is associated with higher LEEP scores.

%\tm{Suggestion: Already use subscript $s$ to denote the source, so use $\mathcal{Z}_s$ an $\textrm{LEEP}_s$, that makes extensions in the next paragraph(s) even more clear.}\jasper{I see what you mean, but I am not fully convinced about the trade-offs. Let's discuss.}


\subsection{Multi-source selection transferability metrics} \label{metric-multi-source}
%\subsection{Transferability metrics for multi-source selection} \label{metric-multi-source}
%\subsection{Transferability metrics for multi-source selection} \label{metric-multi-source}

We design four transferability metrics suitable for multi-source selection.
We base all our approaches on the EEP predictor \eqref{eq:eep}, which provides a mathematical foundation to establish relationships between source models.
In all cases our ensembles contain a fixed number $S$ of source models.

\para{Multi-Source LEEP (MS-LEEP).}
A natural way of extending LEEP to the multi-source setting is to compute the joint probability distribution over the $S$ source model predictions, where each model makes predictions in its own label space.
%
%We define a new empirical conditional distribution for a target label $y$, given the labels $z_s$ predicted by each source $s$ \jasper{the following equation seems unnecessary. Andrea, please fix.}
%
%\begin{equation}
%    \hat{P}(y|z_1,z_2,\dotsm,z_S) = \frac{\hat{P}(y,z_1,z_2,\dotsm,z_S)}{\hat{P}(z_1,z_2,\dotsm,z_S)}
%   \label{eq:exact_multi_source_cond_distribution}
%\end{equation}
%
% To be useful for guiding the selection of source models, 
But this requires calculating the joint probability distribution for every possible subset of $S$ models, which is infeasible for a large pool of $N$ models.
%
Instead, we assume the source models to be independent, yielding a simplified joint conditional distribution:
%
\begin{equation}
%    \hat{P}(y|z_1,z_2,...,z_S) \approx \prod_{s=1}^{S}{\frac{\hat{P}(y,z_s)}{\hat{P}(z_s)}} = \prod_{s=1}^{S}{\hat{P}(y|z_s)}
    \hat{P}(y|z_1,z_2,...,z_S) \approx  \prod_{s=1}^{S}{\hat{P}(y|z_s)}
    \label{eq:proxy_multi_source_cond_distribution}
\end{equation}
%
We extend \eqref{eq:leep} by applying \eqref{eq:proxy_multi_source_cond_distribution} to define a new metric:
%
\begin{equation}
    \begin{split}
    \mathrm{MS{-}LEEP} & = \frac{1}{n} \sum_{i=1}^{n} \log \left( \prod_{s=1}^{S}\left({\sum_{z_s\in \mathcal{Z}_s}{\hat{P}(y_i|z_s) p_{\textrm{s}}(z_s|x_i)}}\right)\right) \\ & = \frac{1}{n} \sum_{i=1}^{n} \left(\sum_{s=1}^{S}{\log p_s(y_i|x_i)}\right) = \sum_{s=1}^{S}{\mathrm{LEEP}_s}    
        \label{eq:p-leep}
    \end{split}
\end{equation}
%When assuming the source models to be independent, the computation reduces to the sum of the individual LEEP scores of each source.
%
Hence MS-LEEP can be seen as taking the best source models according to the single-model metric LEEP. This suggests that other existing transferability metrics~\cite{bao19icip, li21cvpr, you21icml, tran19iccv} can be similarly adapted to ensemble selection.


\para{Ensemble LEEP (E-LEEP).}
We now approach the problem from a different prospective, stressing that we want to predict the transfer performance of an {\em ensemble} of models.
For this we consider the ensemble prediction as the average of the $S$ individual models predictions.
Considering \eqref{eq:eep} as a single-source predictor $p_s(y_i|x_i)$, we can construct the prediction of the ensemble as
%
\begin{equation}
p_{\textrm{ens}}(y_i|x_i) = \frac{1}{S}\sum_{s=1}^{S} p_s(y_i|x_i)
\label{eq:ensemble-predictor}
\end{equation}
%
By reformulating \eqref{eq:leep} accordingly, we get a new metric:
%
\begin{equation}
  \mathrm{E{-}LEEP} = \frac{1}{n}\sum_{i=1}^{n}\log p_{\textrm{ens}}(y_i|x_i)
  \label{eq:e-leep}
\end{equation}
The difference with \msleep{} \eqref{eq:p-leep} is the order of the log and the sum: \eleep{} uses the log of the mean predictions, while \msleep{} uses the mean of the log predictions.

\para{IoU-EEP.} \label{iou-eep}
While \msleep{} and \eleep{} estimate pixel classification accuracy, semantic segmentation performance is usually measured as Intersection-over-Union (IoU).
In practice, for IoU we count True Positives (TP), False Positives (FP), False Negatives (FN), and calculate $\frac{TP}{TP + FP + FN}$.
IoU is calculated separately per class, and then averaged into a single metric (mean IoU).
\begin{comment}
It measures the area of intersection between the predicted and the ground-truth mask of a class, divided by the area of their union.
\end{comment}
In order to design a transferability metric that more directly approximates mean IoU, we first use the ensemble predictor \eqref{eq:ensemble-predictor} to compute the predicted semantic segmentation over the target training set
%
\begin{equation}
  y_i^* = \arg\max_{y \in \mathcal{Y}} p_{\textrm{ens}}(y|x_i)
  \label{eq:e_eep_argmax}
\end{equation}
%
where $y$ now iterates over the entire target label space (as opposed to being the one ground-truth label $y_i$). 
Finally, we use these predictions $y_i^*$ to calculate the mean IoU, arriving at the \ioueep{} transferability metric.
%
This metric is also less dependent on the probabilistic output of the source classifiers, which are often poorly calibrated \cite{guo17icml} and therefore could negatively affect the metric.

\para{SoftIoU-EEP.} \label{soft-iou-eep}
Applying the $\arg\max$ in Eq.~\eqref{eq:e_eep_argmax} alleviates calibration errors. But it also loses the fine-grained information in the probability distribution $p_{\textrm{ens}}(\cdot|x_i)$, which could be helpful in ranking similar models.
%
Hence, we propose to introduce a "Soft-IoU" relaxation. For every pixel $x_i$, instead of counting True Positives, we aggregate their confidences $p_{\textrm{ens}}(y_i|x_i)$ (where $y_i$ is the ground-truth label of that pixel). Therefore the higher the confidences of correct predictions, the higher the predicted transferability.
We do the analogue for errors (FP and FN) by aggregating $1 - p_{\textrm{ens}}(y_i|x_i)$. Since errors are in the denominator, the higher their confidences the lower the predicted transferability.
%
\begin{comment}
Hence, we propose to introduce a "Soft-IoU" relaxation, where we assign a weight to every pixel $x_i$.
%\tm{is it a mathematical relaxation?}
%\vitto{maybe not as we are not softening a constraint, but it sounds like a good word here anyway}
This weight is either its prediction probability $p_{\textrm{ens}}(y_i|x_i)$ when the model is correct ($y_i^*=y_i$), or $1 - p_{\textrm{ens}}(y_i|x_i)$ when the model is incorrect (where $y_i$ is the ground-truth label of that pixel).
\end{comment}
%
%\tm{Why soft and not weighted? From the current description it seems that just weights are added to each pixel prediction (which could be handled by keras MeanIoU.} \andrea{to reply also to the other comment, yes, I actually use the weighted version of keras Mean IoU, the relaxation is in terms of the confusion matrix, basically in keras they compute mean iou from the confusion matrix, and the weights are given to the function that computes the confusion matrix, basically instead of counting you sum the weights}








%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%% OLD 3.0 FROM HERE.
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\andrea{Now I state the task definition we are solving, and introduce what a transferability metric is. I define on which sets we train and evaluate. I dont have a figure yet, but if it is needed also with this new introduction I can do it.}
\vitto{it is needed. In general you need figures in a paper. This paper has now zero figures! You need to illustrate your work. Schemes with bubbles and arrows, such stuff.}
\andrea{Done}

\jasper{Made opening sentence more generic: earliest methods did no do source model selection.}
Transferability metrics were introduced to efficiently determine how well a source model would perform on a target task in a transfer learning setting, primarily applied to classification tasks~\cite{nguyen20icml, you21icml, tan21cvpr, li21cvpr}.
% ORIGINAL VITTO TEXT: Transferability metrics were introduced for doing \andrea{yes in general, but actually the first ones, h score and nce didnt do source selection, what about saying smth like 't.m. are used for doing' or 'applied to'?} source model selection for transfer learning, primarily applied to classification tasks~\cite{nguyen20icml, you21icml, tan21cvpr}. 
In the standard setting, we are given $N$ source models, and a target dataset \andrea{removed $D$ as we dont really need it here, but later}. The source models are usually constructed by training different model architectures on a single source dataset \cite{nguyen20icml, you21icml, li21cvpr}, or by training the same architecture on different source datasets \cite{tan21cvpr, li21cvpr}.
%
The goal is to select a single source model which, after fine-tuning on the target training set, yields the best performance on the target test set. Since fine-tuning all $N$ source models on the target training set is too computationally expensive, the main idea is to predict future performance using a computationally efficient transferability metric.
\vitto{much better now, well done! However, the notion of where the pre-trained source models could ever come from is too mysterious now. You need to give a feeling, just a few words, e.g. 'pre-trained on different source datasets, or with diff archys, or training schemes, whatever'. This opening should be a mini-world of your whole section.}
\andrea{Done, but maybe there is a shorter way}
Instead, we aim to select an \emph{ensemble} of $S$ source models.
%which, after fine-tuning on the target training set, yields the best ensemble performance on the target test set.
This is arguably a more challenging scenario since the number of possible ensembles grows w.r.t. the binomial coefficient $\binom{N}{S}$ \vitto{pretty argument but mathematically imprecise: it's not a factorial, it's a binomial coefficient (n choose k)}.\andrea{done, defined $S$ before}
%
Additionally, we construct source models by training combinations of different pre-trained model architectures on multiple source datasets. \andrea{here I merge the pre-trained concept on model architectures so we can compare to the previous works (archi + training on source dataset)}
%
Finally \vitto{nope, you should say the prev work is for classification in the opening para, then say here you tacke the more complex sem segm task.} \andrea{done}, we address the more complex semantic segmentation task, where instead of having a single label per image, we have predictions at every pixel.
%
These changes significantly increase computational complexity. \vitto{wrong point to tell this detail. Suddenly LEEP comes up, with no contextualization about what it could be. And the section on it is in 1.5 pages! Just don't say it here.} \andrea{removed LEEP}

We first describe in \cref{preparing_source_models} the preparation of a pool of $N$ diverse source models
%, where we exploit 3 factors of diversity such as model architecture, image domain and pre-training strategy
\vitto{this concept has to appear earlier, in the opening para, as a concept to show how could you ever have different source models (with concrete examples from previous papers only). Then in 3.1 you detail what are YOUR factors of diversity}. \andrea{done}
Then, \cref{metric-semantic-segmentation} presents a solution to compute a transferability metric for the computationally expensive semantic segmentation task. \cref{leep-single} describes LEEP \cite{nguyen20icml}, a single-source selection metric that we use as starting point for our 4 transferability metrics that can be applied to the multi-source selection setting (\cref{metric-multi-source}).
\end{comment}

==> Transferability Metrics for Selecting Source Model Ensembles- CVPR 2022/4_transferability_metrics.tex <==
\section{Evaluating transferability metrics} \label{sec:evaluate-metrics}

\subsection{Experimental setup} \label{multi-source-exp-setup}

The standard procedure to evaluate transferability metrics is to consider several candidate source models for a given target dataset, and measure the correlation between
(A) the transferability score and
(B) the actual performance on the target test set after the source model has been fine-tuned on the target training set~\cite{nguyen20icml, li21cvpr, tan21cvpr, you21icml}. 

In this paper we consider multiple candidate source model \emph{ensembles} for a given target dataset. To measure the desired correlation, we calculate transferability as in Sec.~\ref{metric-multi-source} and we also need to calculate the actual performance of each ensemble on the target dataset.

Considering ensembles leads to additional computational challenges. The number of possible ensembles of $S$ source models out of a pool of $N$ is very large
(the binomial $\binom{N}{S}$). Hence computational efficiency is an important requirement in our experimental design.


\para{Measuring actual performance of ensembles efficiently.}
Given a candidate ensemble, we fine-tune each member model individually and apply it individually on the target test set. Then we take the average of their predictions as the ensemble prediction.
Finally, we measure actual ensemble performance as mean IoU.
%
By considering the predictions of each ensemble member individually, we can reuse them across ensembles. Hence, we only need to run inference for each model on a target test sample {\em once}, regardless of the number of ensembles the model participates in.

While it would also be possible to fine-tune each ensemble as a whole, this is too computationally expensive for this experiment. We do it in a different setting in Sec.~\ref{sec:ensemble_selection}.

\para{Ensemble size.}
We fix the number of models in an ensemble to $S=3$. We found $S=3$ to be a good compromise to benefit from a diverse ensemble, while limiting overall computation (more details in the Appendix C). %\vitto{ALERT. Make it Appendix}.
%This is a good compromise to benefit from a diverse ensemble, while limiting overall computation \jasper{(See Appendix XX)}.
% with $N=15$ and $S=3$, the total number of possible ensembles is 455.

\para{Subsampling candidate source models.}
For a given target dataset, the total number of candidate source models is 64 (68 minus the 4 trained on that target).
We reduce the number of candidates to gain two types of speed-ups.
Firstly, this requires fine-tuning fewer source models on the target training set.
But more importantly, the number of candidate ensembles grows factorially with $N$: for $N=64$ and $S=3$ there are 41k possible ensembles. While this is not a problem for calculating our transferability metrics, evaluating the performance of 41k ensembles on the target test set is computationally prohibitive.
Hence we limit $N=15$ as described below, yielding $455$ candidate ensembles.

For each target dataset we sample 15 source models as follows. As the final goal is to select a high-performing ensemble, we pick 5 good source models for that target. We first compute all our transferability metrics for all ensembles of $3$ source models from the complete pool ($N=64$). We then select the 5 most frequent models in the top-ranked ensembles across all metrics. 
Since we want to evaluate the ability to distinguish between good and bad sources, we include an additional 10 source models at random.


\para{Target datasets.} We consider five target datasets: Cam\-vid~\cite{brostow09prl}, ISPRS~\cite{rottensteiner14isprs}, vKITTI2 \cite{cabon20arxiv}, KITTI \cite{alhaija18ijcv} and Pascal VOC \cite{everingham12pvoc}. 
Since transfer learning is particularly interesting in scenarios with limited training images~\cite{kolesnikov20eccv,mensink21arxiv,mustafa20arxiv}, we follow \cite{mensink21arxiv} and limit each target training set to 150 images.

\para{Correlation measure: weighted Kendall Tau.}
A transferability metric is useful when it can order the candidate source models (or ensembles) according to their actual performance. The exact predicted performance value is less important.
Therefore we use a rank correlation measure as in~\cite{li21cvpr, mensink21arxiv}. Moreover, as in practice we mainly care about selecting a high performing ensemble, we follow~\cite{you21icml} and use a weighted version of Kendall $\tau$ considering top-ranked items more important than low-ranked ones~\cite{vigna15www}.


\para{Baseline transferability metric.}
As there is no previously proposed transferability metric for source model ensembles, we introduce a simple baseline. It is  based on three factors:
(1) source model performance $P_s$ evaluated on a source test set,
(2) source dataset size $N_s$ in terms of number of images, and
(3) source dataset richness measured by the number of source classes $C_c$.
For a candidate ensemble containing $S$ source models, we calculate this baseline as:
$\mathrm{BASE} = \sum_{s=1}^{S}(P_s \times N_s \times C_s)$.
%
%\begin{equation}
%    \mathrm{BASE} = \sum_{s=1}^{S}(P_s \times N_s \times C_s)
%\end{equation}
%
This baseline is target-agnostic, favours broad source datasets (COCO, ADE20k, Mapillary), and the best model architecture (HRNetV2-W28, pre-trained fully supervised; as it typically leads to higher $P_s$).

\begin{figure}[t]
\vspace{-.8cm}
  \includegraphics[width=8cm]{figures/scatterplot_transferability_metrics_few_targets.pdf}
  \centering
   \caption{
   Relation between the predicted transferability (y-axis) and the actual mean IoU performance (x-axis) on the target test set (for 2 of the 5 target datasets). Each plot shows 455 candidate ensembles as a separate dot, and also reports the corresponding weighted Kendall's $\tau$ correlation score.
   These scores are generally high, demonstrating the success of our transferability metrics.}
   \label{fig:scatterplot_transferability_metrics}
   \vspace{-.4cm}
\end{figure}


\subsection{Results} \label{correlation-results}

\cref{fig:scatterplot_transferability_metrics} shows qualitatively the relation between predicted transferability and actual mean IoU for all our transferability metrics on two target datasets.
In all experiments we see good positive correlations, demonstrating that our metrics work well.
We also see that ensemble performance varies greatly depending on the sources used, justifying the importance of having a good ensemble selection mechanism.

Quantitatively, \cref{fig:comparison_transferability_metrics} reports the weighted Kendall's $\tau$
for our transferability metrics and the baseline (for all 5 target datasets). All our transferability metrics generally achieve high scores, significantly outperforming the baseline on each target dataset.
%
Among our metrics, the direct LEEP variants, MS-LEEP and E-LEEP, perform equally well.
%
Next, IoU-EEP performs the worst, suggesting that it is important to consider the probability distribution $P_{ens}(\cdot|x_i)$.
%
Finally, \softiou{} performs best, confirming the benefits of directly approximating the performance measure of the target test set (mean IoU).
%
On average, \softiou{} achieves $\tau$ of 69.3\%, outperforming the baseline by 20.3\%, \msleep{} by 3.1\%, \eleep{} by 3.6\%, \ioueep{} by 8.4\%.

\begin{figure}[t]
\vspace{-.7cm}
  \includegraphics[width=7.0cm]{figures/transferability_metrics_comparison.pdf}
  \centering
   \caption{Comparison of our transferability metrics, over 5 target datasets. We show the weighted Kendall's $\tau$ between a metric and actual mean IoU on the target test set, where each ranks all 455 candidate ensembles. \softiou{} performs best overall.}
   \label{fig:comparison_transferability_metrics}
   \vspace{-.4cm}
\end{figure}

As related works on single-source transferability metrics sometimes report the standard Kendall $\tau$~\cite{li21cvpr} or the (linear) Pearson coefficient~\cite{tan21cvpr,nguyen20icml, li21cvpr}, we also report them in \cref{tab:correlation_measures}. Despite each correlation measure is based on different mathematical assumptions, the general trend among target datasets and transferability metrics remains the same.

\begin{table*}
\vspace{-.8cm}
\small
  \centering
  \begin{tabular}{c|*{5}{@{\hspace{3.5mm}}c}|*{5}{@{\hspace{3.5mm}}c}|*{5}{@{\hspace{3.5mm}}c}}
    \toprule
    Measure & \multicolumn{5}{c}{Weighted Kendall's $\tau$} & \multicolumn{5}{c}{Kendall's $\tau$} & \multicolumn{5}{c}{Pearson} \\
    %Method & MS-L. & E-L. & IoU-E. & S.IoU-E. & MS-L. & E-L. & IoU-E. & S.IoU-E. & MS-L. & E-L. & IoU-E. & S.IoU-E.\\
    Method & BASE & MS & E & IoU & sIoU & BASE & MS & E & IoU & sIoU & BASE & MS & E & IoU & sIoU\\
    \midrule
    Camvid & 0.51 & 0.69 & \textbf{0.70} & 0.50 & 0.68 & 0.30 & \textbf{0.56} & 0.55 & 0.37 & 0.51 & 0.46 & \textbf{ 0.74} & 0.73 & 0.56 & 0.70\\
    ISPRS & 0.45 & 0.61 & 0.54 & 0.59 & \textbf{0.68} & 0.22 & 0.41 & 0.37 & 0.41 & \textbf{0.44} & 0.29 & 0.60 & 0.55 & 0.59 & \textbf{0.63}\\
    vKITTI2 & 0.56 & 0.57 & 0.58 & \textbf{0.60} & \textbf{0.60} & 0.38 & 0.49 & 0.51 & 0.51 & \textbf{0.53} & 0.54 & 0.66 & 0.67 & 0.62 & \textbf{0.70}\\
    KITTI & 0.22 & 0.62 & 0.65 & 0.54 & \textbf{0.66} & 0.17 & 0.50 & \textbf{0.54} & 0.42 & 0.53 & 0.25 & 0.69 & 0.73 & 0.62 & \textbf{0.74}\\
    PVOC  & 0.71 & 0.81 & 0.82 & 0.81 & \textbf{0.83} & 0.42 & 0.59 &\textbf{ 0.61} & 0.58 & \textbf{0.61} & 0.66 & \textbf{ 0.84} & 0.83 & 0.73 & 0.81 \\
    \bottomrule
    Average & 0.49 & 0.66 & 0.66 & 0.61 & \textbf{0.69} & 0.30 & 0.51 & \textbf{0.52} & 0.46 & \textbf{0.52} & 0.44 & 0.71 & 0.70 & 0.62 & \textbf{0.72}\\
  \end{tabular}
  \caption{Correlation measures for 5 different target datasets, obtained by comparing the transferability predicted by a metric to the actual Mean IoU on the target test set. The methods shortcuts refer to: (BASE=Baseline), (MS=\msleep{}), (E=\eleep{}), (IoU=\ioueep{}), (sIoU=\softiou{}). \softiou{} performs best overall. See Sec. \ref{multi-source-exp-setup} for more details about the setup.}
  \label{tab:correlation_measures}
  \vspace{-.4cm}
\end{table*}



==> Transferability Metrics for Selecting Source Model Ensembles- CVPR 2022/5_ensemble_selection.tex <==
\section{Evaluating ensemble selection} \label{sec:ensemble_selection}

% Most works on transferability metrics consider transferring from a single model \cite{you21icml, nguyen20icml, bao19icip, tran19iccv}. This is a viable alternative we compare against. In the previous section we validated our transferability metrics, with Soft-IoU$_{EEP}$ as the most predictive of transferability. Here we make use of all 68 source models available, and we test our selected ensembles against a single model baseline.

\subsection{Experimental Setup} \label{sec:ensemble_selection_setup}

We now turn to ensemble selection: we use our best transferability metric, \softiou{}, to select the ensemble with the highest predicted transferability. We fine-tune this ensemble on the target training set and evaluate on the target test set.
Selecting only a single ensemble per target dataset on which to perform expensive fine-tuning and evaluation enables us to expand our experimental setup beyond what we did in Sec.~\ref{sec:evaluate-metrics}. Instead of using $N=15$, we now use all $N=64$ source models as candidates. Moreover, instead of only fine-tuning individual ensemble members, we add an additional step of ensemble-specific fine-tuning.
%
We compare to two baselines which select a single source model.

% PRE CAMERAREADY
% We now turn to ensemble selection: we use our best transferability metric, \softiou{}, to select the ensemble with the highest predicted transferability. We then fine-tune this ensemble on the target training set and evaluate on the target test set.
% Selecting only a single ensemble per target dataset on which to perform the expensive fine-tuning and evaluation operations enables us to expand our experimental setup beyond what we did in Sec.~\ref{sec:evaluate-metrics}. Instead of using just $N=15$, we now use all $N=64$ source models as candidates. Moreover, instead of only fine-tuning individual ensemble members, we add an additional step of ensemble-specific fine-tuning.
% %
% We compare to two baselines which select a single source model.

\para{Improved actual performance of ensembles.}
Given an ensemble, we start by fine-tuning each member individually on the target training set as in Sec.~\ref{multi-source-exp-setup}.
Afterwards, we perform additional ensemble-specific fine-tuning to improve it by re-weighting the class predictions of its members.
Specifically, we freeze the backbone of each member and attach to it a light head that assigns per-class weights and biases, before averaging their predictions into a single ensemble prediction.
We then fine-tune the light head of this ensemble on the target training set.
%
While the total number of additional parameters introduced by this head depends on the number of target classes, in practice it is between 144 and 2700, which is negligible compared to the total number of parameters in the models composing the ensemble.
 
%For each source model, that produces the logits $logits_s(x)$, we add the following computation:
%\begin{equation}
%    logits_s(x) = Relu\left(logits_s(x) \vec{w} +\vec{b}\right) + logits_s(x)
%    \label{eq:finetune_ensemble_block}
%\end{equation}
%where $\vec{w} = [w_1, w_2 \dotsm w_{NC}]$ are per class weights and $\vec{b} = [b_1, b_2 \dotsm b_{NC}]$ per class biases, with $NC$ representing the total number of target classes \vitto{use a single letter for this, otherwise it looks like $N$ times $C$}. We apply \cref{eq:finetune_ensemble_block} sequentially 3 times, before averaging together the predictions of the source models. \vitto{this whole explanation is way too complicated and I really don't get it}

\para{Ensemble size.} We set $S=3$ as in Sec.~\ref{sec:evaluate-metrics}. 

\para{Target datasets.} 
We now consider each of the 17 datasets in~\cref{tab:datasets} as a target dataset in turn (instead of 5 in Sec. \ref{sec:evaluate-metrics}).
As in Sec.~\ref{sec:evaluate-metrics}, we study transfer learning in the low data regime defined by~\cite{mensink21arxiv} (i.e. 150 target training images for each dataset, except 1000 for COCO and ADE20k as they contain many classes).

\para{Baseline B1: select a single source model.}
We test whether aggregating multiple source models is beneficial to transfer learning, compared to the standard of selecting a single source model~\cite{nguyen20icml, li21cvpr, tan21cvpr, you21icml}.
%
To do so, for a given target dataset we use the same pool of 64 source models as for ensemble selection. Then we select the single model with the highest predicted transferabiliy according to LEEP~\cite{nguyen20icml}. Finally, we fine-tune it on the target training set, and evaluate on the target test set.


\para{Baseline B1L: select a single \emph{large} source model.} \label{para:single-model-finetuning}
We also propose a stronger baseline which selects a single large model with the same number of parameters as one of our ensembles. An ensemble of $S=3$ has 69M parameters, as both HRNetV2-W28 and ResNet23M have 23M parameters.
We use the best such model according to preliminary experiments: HRNetV2-W48 pre-trained fully supervised on ILSVRC'12.
It offers excellent performance for semantic segmentation~\cite{wang20pami} and was also used in~\cite{lambert20cvpr, mensink21arxiv}.

For this baseline we need to construct a new pool of large source models. To do so, we train 17 large models, one for each source dataset (Tab. \ref{tab:datasets}). Then, given a target dataset, we use LEEP~\cite{nguyen20icml} to select a single model (out of 16, excluding that target dataset).


\begin{comment}
We perform transfer learning by selecting a single large source model from a pool of possible source models using a transferability metric.
%~\cite{you21icml, nguyen20icml, bao19icip, tran19iccv}.
However, for a fair comparison, it should have the same number of parameters as the total sum of parameters in the $S=3$ models composing one of our ensembles (69M as both HRNetV2-W28 and ResNet23M have 23M parameters).
We use the best such model according to preliminary experiments: HRNetV2-W48 pre-trained fully supervised on ILSVRC'12.
It offers excellent performance for semantic segmentation~\cite{wang20pami} and was also used in~\cite{lambert20cvpr, mensink21arxiv}.

We carry out transfer learning with this large model backbone as follows. First we train 17 large source models, one on each source training set.
Given a target dataset, we then select a single source model using LEEP~\cite{nguyen20icml} (out of a pool of 16 models, as we exclude the target dataset itself).
Finally, we fine-tune the selected source model on the target training set.
\end{comment}


\subsection{Results} \label{sec:ensemble_selection_results}

\begin{figure}[t!]
  \vspace{-.1cm}
  \includegraphics[width=8cm]{figures/soft_iou_vs_baselines.png}
  \centering
   \caption{Relative mean IoU gain on each target test set made by the ensemble selected by our \softiou{} metric over baseline B1L.
   % which selects a single large source model by LEEP. 
   For clarity, we set the 0 vertical line to corresponds to the performance of B1L. On average over all target datasets, the improvement is 2.5\%.
   We do not explicitly display baseline B1, as it performs worse than B1L (see main text for discussion).
   }
   \label{fig:ensemble_vs_baseline_relative_gain}
   \vspace{-.4cm}
\end{figure}

\begin{figure*}[t]
    \vspace{-.8cm}
  \includegraphics[width=16cm]{figures/ensemble_selected_soft_iou.pdf}
  \centering
   \caption{For each target dataset (x-axis), we show the 3 source models in the ensemble selected by \softiou{}. When multiple source datasets cover the image domain of the target, our metric generates diversity by selecting models trained on these different source datasets (see target ScanNet and Sun). When there exists a single strong source dataset for a target, our metric selects only this source dataset, and instead generates diversity by varying architectures and pre-training schemes (see targets from the driving domain).
   Note: we do not consider source models trained on the same dataset as the target (gray cells).
   }
   \vspace{-.3cm}
   \label{fig:soft_iou_selected_ensembles}
\end{figure*}

\para{Comparison to baselines B1 and B1L.}
We first consider the improvement made by the ensemble selected by our transferability metric \softiou{} over the baseline B1.
On average across all 17 dataset, selecting an ensemble instead of a single model out of the same pool (B1) improves results by a relative +6.0\% mean IoU. This demonstrates that the source models in our pool are complementary and composing several into an ensemble brings clear benefits.

Next, we show in Fig.~\ref{fig:ensemble_vs_baseline_relative_gain} that
selecting an ensemble out of our pool even outperforms baseline B1L, which selects a single model out of a pool of {\em larger models}, each with capacity similar to one of our ensembles (+2.5\% relative mean IoU).
When looking at individual target datasets,
the selected ensemble improves over B1L by more than 2\% in 10 of them.
In contrast, B1L outperforms the ensemble only once (on Pascal Context).
We conclude that selecting an ensemble brings solid accuracy benefits over selecting a single model, even when controlling for total capacity.

%%%%%%%% TABLE WITH ABSOLUTE mIOU GAINS.
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|ccc}
%     \toprule
%          & Ensemble & B1 & B1L \\
%     average mIoU & 0.470 & 0.445 & 0.460 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Average mean IoU (mIoU) over all 17 datasets.}
%     \label{tab:comparison_single_model}
% \end{table}
% 


% \para{Comparison with single model baselines.} \andrea{Variation considering both baselines}
% \cref{fig:ensemble_vs_baselines_relative_gain} compares the performance of the selected ensemble (using \softiou{}) against the baselines B1 and B1L, which both use LEEP to select a single-source model \andrea{I am assuming I put both results in the figure, maybe as subplots}. When using the same pool of source models, the selected ensemble outperforms the selected single-source on every target dataset. On average across all datasets, the ensembles outperform B1 by 6\% mean IoU. 
% 
% Additionally, the selected ensemble outperforms the single large baseline B1L by more than 2\% mean IoU in 10 out of 17 target datasets. In contrast, B1L outperforms the ensemble only once, for Pascal Context.
% On average across all datasets, the ensembles outperform B1L by 2.5\% mean IoU.
% 
% \andrea{Next sentence is probably a candidate for the conclusion if here we want to leave just the results}
% This shows that aggregating multiple source models selected by our transferability metric is beneficial over the standard of selecting a single source model, even when the single model is selected from a stronger pool of large source models (B1L).
% 
% \para{Comparison with single large baseline.} \andrea{Old para for large baseline}
% 
% \cref{fig:ensemble_vs_baseline_relative_gain} compares the performance of the selected ensemble with the baseline of selecting a single model. As can be seen, \softiou{} metric outperforms the baseline by more than 2\% mean IoU in 10 out of 17 target datasets.
% In contrast, the baseline outperforms the ensemble only once, for Pascal Context.
% %, and they are within 2\% on 6 datasets.
% On average across all datasets, the ensembles outperform the baseline by 2.5\% mean IoU.



% \begin{figure}[h!]
%   \includegraphics[width=8cm]{figures/soft_iou_vs_both_baseline_subplot.pdf}
%   \centering
%    \caption{Test for how to put both figures. \andrea{Do you prefer something like this or separate figures? Or do we show just B1L?}}
%    \label{fig:ensemble_vs_baselines_relative_gain}
% \end{figure}

%
\para{What factors of diversity matter more?}
Generally, ensembles benefit from the predictive diversity of its member models \cite{bian21ieee, dietterich00springer, lu10sigkdd, guo18neurocomp}.
To understand which factors of diversity are important in our transfer learning setting (Sec. \ref{preparing_source_models}), \cref{fig:soft_iou_selected_ensembles} shows which source models are selected by \softiou{} as part of the winning ensemble for each target dataset.

We observe the following patterns:
(1) Some target datasets are well covered by multiple source datasets. For these cases, our metric generates diversity by selecting source models trained on these different datasets. For example, for ScanNet (indoor) as a target, our metric selects source models trained on Sun (indoor), COCO, and ADE20K, as COCO and ADE20K contain many indoor images.
In these cases the backbone of choice is HRNetV2-W28 using fully supervised pre-training, which is generally the best perfoming backbone (76\% of all source models selected).
(2) For other target datasets there exists a strong source dataset which alone already covers most variations in the target domain. For example, Mapillary is the largest dataset in the driving domain and covers all continents. Our method nicely picks Mapillary almost exclusively as the sole source dataset for all target driving datasets (Cityscapes, IDD, BDD, Camvid, vKITTI2, and KITTI as the only case with a second source - Cityscapes).
In these cases, our metric generates diversity by varying model architectures and pre-training schemes within the selected ensemble.
(3) The most frequently selected source datasets have a greater number of training samples, greater number of labels, and larger diversity of images (Mapillary, COCO, ADE20K).
%
These observations are in line with earlier work which show the benefits of in-domain source images~\cite{ngiam18arxiv, mensink21arxiv, yan20cvpr} and large, broad source sets~\cite{kolesnikov20eccv, mahajan18eccv, mensink21arxiv, sun17iccv}.


%\jasper{Maybe give an explicit example, now commented out in the tex.}
% When the target image domain is contained within the source dataset, the selected ensemble exploits other factors of diversity such as pre-training strategy and backbone architecture, as for Mapillary used as source for other driving datasets. The most frequent source datasets selected are the ones with the highest number of training examples and wider range of diverse images. In fact, for cases with no strong in-domain other source, such as for SUIM and iSAID, COCO and ADE20K are the only sources used to combine ensembles. Combinations of the latter observations can be seen for the Indoor target datasets, SUN and Scannet. They take advantage of the other in-domain source dataset, while also exploiting general good sources such as COCO and ADE20K, using the most performing pre-training strategy (supervised) and backbone (HRNet).

\para{Ensemble vs. its members.}
In \cref{fig:single_sources_vs_ensemble_eleep} we compare the mean IoU of the selected ensemble to that of its member models. On average the ensemble improves over its best member by 4.6\%, and over its worst member by 18.6\%.
%
These improvements demonstrate that the sources selected to be part of the winning ensemble are indeed diverse (otherwise the ensemble could not outperform its best member).
Hence we conclude that our transferability metric is good in selecting a diverse set of source models.

\begin{figure}[t]
  \includegraphics[width=8cm]{figures/single_sources_vs_ensemble_eleep.pdf}
  \centering
   \caption{Comparison of the mean IoU of the winning ensemble vs its component source models.}
   \label{fig:single_sources_vs_ensemble_eleep}
   \vspace{-.3cm}
\end{figure}

Finally, to evaluate how important it is to \emph{learn} to combine model predictions, we re-evaluate the results but now using a simple unweighted average of the model predictions instead of the learned head. This still outperforms the best single ensemble member by +2.9\%.  %(vs +4.6\% for the learned head, L.802-805).
%
Hence, our improvements are truly due to ensembling models (be it with a fixed combiner head, or with a learned one).








%%%%%%%%%%%%%%%%%%%%%
%%%%%%% OLD VERSION
%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\subsection{OLD version of: Preparing ensembles and single model baselines}



\para{Fine-tuning the ensemble.} \label{para:ensemble_finetuning}
As explained in \cref{multi-source-exp-setup}, for each of the 17 target datasets, we have 64 possible source models to transfer from. We apply Soft-IoU$_{\mathrm{EEP}}$ using each source model applied to the target training set, and we select the ensemble of 3 source models with the highest transferability score. We do this for each of the 17 target datasets. Compared to \cref{sec:evaluate-metrics}, in this setup we only fine-tune and evaluate a single ensemble, for each target dataset. Therefore, to improve performance, after fine-tuning independently the source models on the target training set, we also train an extra head for each ensemble. More specifically, we first freeze the backbones of each source model and attach a light head that assigns per class weights and biases, for each source model. We train the new heads jointly again on the target training set. The total count of additional parameters depends on the number of target classes, in practice the parameters vary between 144 and 2700 depending on the dataset, which is negligible compared to the total size of the ensemble.
 
%For each source model, that produces the logits $logits_s(x)$, we add the following computation:
%\begin{equation}
%    logits_s(x) = Relu\left(logits_s(x) \vec{w} +\vec{b}\right) + logits_s(x)
%    \label{eq:finetune_ensemble_block}
%\end{equation}
%where $\vec{w} = [w_1, w_2 \dotsm w_{NC}]$ are per class weights and $\vec{b} = [b_1, b_2 \dotsm b_{NC}]$ per class biases, with $NC$ representing the total number of target classes \vitto{use a single letter for this, otherwise it looks like $N$ times $C$}. We apply \cref{eq:finetune_ensemble_block} sequentially 3 times, before averaging together the predictions of the source models. \vitto{this whole explanation is way too complicated and I really don't get it}
\para{The single model baseline.} \label{para:single-model-finetuning}
%
\jasper{Again: goal is missing. Why this baseline. It goes immediately in-depth}
In preliminary experiments, supervised pre-trained HRNet resulted to be the best combination of pre-training strategy and model architecture, when trained on the source datasets. Therefore, in our single model baseline we decide to start with HRNet, with supervised pre-trained weights on ILSVRC'12. For fair comparison, we use HRNetV2-W48, a large single model which consists of 69M parameters, exactly the same of an ensemble of 3 source models. As before, we add a single linear classification layer to the backbone. We follow the same training procedure as \cref{para:training-setup} to train the large single model on the available 17 source training sets, generating 17 possible large source models. Then, we apply the single model transferability metric LEEP, described in \cref{leep-single}, to select the best single models, for each target dataset. Finally, we fine-tune the selected models on the target training sets. This produces 17 single model baselines, one for each target dataset, which we compare against our selected ensembles.

%As an aside, we demonstrate that we use a good implementation of HRNetV2-W48. Therefore we compare to~\cite{lambert20cvpr} who also use HRNetV2-W48 with a linear classifier. In particular, we compare to them on the MSEG versions of five datasets in~\cref{tab:hrnet48_validation}. As can be seen, our results are comparable and we conclude that we have a solid segmentation framework.
%\vitto{this is such an unrelated point, it does not deserve its own setup subsection.}
%\jasper{Maybe move to appendix?}

%\begin{table}
%  \centering
%  \begin{tabular}{c|c|c}
%   \toprule
%   Dataset & MSEG \cite{lambert20cvpr} & Ours\\
%    \midrule
%    BDD & 63.2 & 65.0\\
%   CityScapes & 77.6 & 75.7\\
%   COCO Panoptic & 52.6 & 54.0\\
%    Pascal Context & 46.0 & 47.1 \\
%    ScanNet & 62.2 & 61.9 \\
%    \bottomrule
%  \end{tabular}
%  \caption{Performance comparison of HRNetV2-W48 between \cite{lambert20cvpr} and our implementation, for multiple MSEG datasets. This validates that %our experiments start from a solid semantic segmentation framework.}
%  \label{tab:hrnet48_validation}
%\end{table}

\subsection{OLD Results} \label{sec:ensemble_selection_results}

For both the ensemble and the single model baseline, we measure performance in terms of mean IoU on the target test set.
%
\cref{fig:ensemble_vs_baseline_relative_gain} shows for each target dataset the difference in mean IoU. In particular, numbers indicate the relative mean IoU improvements when using an ensemble instead of a single model baseline. As can be seen, the ensemble outperforms the baseline for most target datasets. To quantify this, the ensemble outperforms the single model by more than 2\% mean IoU for 10 out of 17 target datasets. In contrast, the single model baseline outperforms the ensemble only once, for Pascal Context. Overall, the ensembles obtain an average gain of 2.5\% across all target datasets.

In summary, results show that relying on multiple factors of diversity, selected by applying the transferability metric Soft-IoU$_{\mathrm{EEP}}$, is a powerful and robust alternative to optimizing single large models.

\begin{figure}[t]
  \includegraphics[width=8cm]{figures/soft_iou_vs_baseline.pdf}
  \centering
   \caption{Relative mean IoU gain from using the finetuned ensembles selected by Soft-IoU$_{\mathrm{EEP}}$, against the baseline single large model suggested by LEEP.}
   \label{fig:ensemble_vs_baseline_relative_gain}
\end{figure}

\subsection{OLD What makes it a good ensemble?} \label{sec:ensemble_analysis}
%
It is widely accepted that ensembles benefit from the predictive diversity of each source model \cite{bian21ieee}. In this section we first compare the performance of an ensemble against its individual members. Then, we ascertain which type of diversity is preferred when composing an ensemble. We analyse all the ensembles previously selected by our metric Soft-IoU$_{\mathrm{EEP}}$, for every target dataset.

\para{Ensemble vs. its individual members.}
%
We verify that ensembles really result in gains with respect to their individual members.
In \cref{fig:single_sources_vs_ensemble_eleep} we show the mean IoU of single models and relative ensemble, for each target dataset. The single source models are constructively aggregated across the 17 target datasets. On average the fine-tuned ensemble improves over its best single member by 4.4\%, and over the worst single member by 18.5\%.

These improvements demonstrate that our sources are diverse: when sources are not diverse, the performance of an ensemble does not outperform their individual members. Furthermore, this demonstrates that our transferability metric is good in selecting a diverse set of sources.

\begin{figure}[t]
  \includegraphics[width=8cm]{figures/single_sources_vs_ensemble_eleep.pdf}
  \centering
   \caption{Comparison of the Mean IoU of single source models, against the performance of the finetuned ensemble.}
   \label{fig:single_sources_vs_ensemble_eleep}
\end{figure}


\para{What factors of diversity are preferred?}
From the ensemble selected, shown in \cref{fig:soft_iou_selected_ensembles}, we notice similar patterns across multiple target datasets.
\begin{figure*}[t]
  \includegraphics[width=16cm]{figures/ensemble_selected_soft_iou.pdf}
  \centering
   \caption{Ensembles of 3 source models selected by Soft-IoU$_{\mathrm{EEP}}$, for every target dataset. Generally, when the source dataset contains the target image domain the ensemble exploits diversity using different backbones and pre-training strategies (Mapillary for the driving target datasets). Alternatively, when there is no single main source dataset the ensemble extends its image domain by using multiple source datasets, while using the most performing backbone and pre-training method (supervised HRNet).}
   \label{fig:soft_iou_selected_ensembles}
\end{figure*}
%
When the target image domain is contained within the source dataset, the selected ensemble exploits other factors of diversity such as pre-training strategy and backbone architecture, as for Mapillary used as source for other driving datasets. The most frequent source datasets selected are the ones with the highest number of training examples and wider range of diverse images. In fact, for cases with no strong in-domain other source, such as for SUIM and iSAID, COCO and ADE20K are the only sources used to combine ensembles. Combinations of the latter observations can be seen for the Indoor target datasets, SUN and Scannet. They take advantage of the other in-domain source dataset, while also exploiting general good sources such as COCO and ADE20K, using the most performing pre-training strategy (supervised) and backbone (HRNet).

In summary, we observe that in presence of a single good source dataset, two ResNets and a single HRNet are chosen 83\% of the time. Instead, when more than one source dataset is used, HRNet supervised is widely preferred, contributing for 76\% to the total types of source models selected.

\end{comment}

==> Transferability Metrics for Selecting Source Model Ensembles- CVPR 2022/6_conclusion.tex <==
\section{Conclusion}

We design for the first time transferability metrics for ensemble selection.
We evaluate them in a challenging and realistic transfer learning setup for semantic segmentation, featuring 17 source datasets covering a wide variety of image domain, two model architectures, and two pre-training schemes.
%
We show experimentally that our transferability metrics rank correlate well with actual transfer learning performance. Moreover, our best metric selects an ensemble performing better than two baselines which select a single source model (even after equalizing capacity).


==> Transferability Metrics for Selecting Source Model Ensembles- CVPR 2022/macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Set this boolean to hide/show comments		    	    %
%     if true, it turns the paper into a christmas tree		%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\providetoggle{showcomments}
\settoggle{showcomments}{true} 								%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iftoggle{showcomments}{% Show with comments and old text
    \newcommand{\changed}[1]{\textcolor{blue}{#1}}
    \newcommand{\todo}[1]{\textcolor{blue}{\textbf{TODO:} #1}}
    \newcommand{\resolved}[3][]{\ifstrequal{#1}{resolved}{\textcolor{blue}{RESOLVED:}~\textbf{{\MakeUppercase #2:}}~{#3}}{\textbf{\MakeUppercase #2:}~#3}}
    \newcommand{\andrea}[2][]{\textcolor{ForestGreen}{\resolved[#1]{andrea}{#2}}}
    \newcommand{\vitto}[2][]{\textcolor{red}{\resolved[#1]{vitto}{#2}}}
    \newcommand{\jasper}[2][]{\textcolor{violet}{\resolved[#1]{jasper}{#2}}}
    \newcommand{\tm}[2][]{\textcolor{magenta}{\resolved[#1]{TM}{#2}}}
    \newcommand{\att}[1]{\textcolor{red}{#1}}
}{% Show final version
    \newcommand{\changed}[1]{#1}
    \newcommand{\todo}[1]{}
    \newcommand{\andrea}[2][]{}
    \newcommand{\vitto}[2][]{}
    \newcommand{\jasper}[2][]{}
    \newcommand{\tm}[2][]{}
    \newcommand{\att}[1]{#1}
}
\newcommand{\TM}[2][]{\tm[#1]{#2}}
\newcommand{\DONE}{\done}
\newcommand{\softiou}{SoftIoU-EEP}
\newcommand{\msleep}{MS-LEEP}
\newcommand{\ioueep}{IoU-EEP}
\newcommand{\eleep}{E-LEEP}
\newcommand{\para}[1]{\par\noindent\textbf{#1}}
% \newcommand{\para}[1]{
%     \par\noindent\textbf{#1}
%     %\subsubsection*{#1}
%     %\paragraph*{\textbf{#1}}
% }
